In-silico Feedback Control of a MIMO Synthetic Toggle Switch via Pulse-Width Modulation

The synthetic toggle switch, first proposed by Gardner & Collins [1] is a MIMO control system that can be controlled by varying the concentrations of two inducer molecules, aTc and IPTG, to achieve a desired level of expression of the two genes it comprises. It has been shown [2] that this can be accomplished through an open-loop external control strategy where the two inputs are selected as mutually exclusive periodic pulse waves of appropriate amplitude and duty-cycle. In this paper, we use a recently derived average model of the genetic toggle switch subject to these inputs to synthesize new feedback control approaches that adjust the inputs duty-cycle in real-time via two different possible strategies, a model based hybrid PI-PWM approach and a so-called Zero-Average dynamics (ZAD) controller. The controllers are validated in-silico via both deterministic and stochastic simulations (SSA) illustrating the advantages and limitations of each strategy

==> PIPASW.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{048}[tc][tc]{\matlabtextA }%
\psfrag{049}[bc][tc]{\matlabtextA \begin{tabular}{@{}c@{}}IPTG\\~\end{tabular}}%
\psfrag{046}[tc][tc]{\matlabtextA \begin{tabular}{@{}c@{}}~\\Time (h)\end{tabular}}%
\psfrag{047}[bc][tc]{\matlabtextA \begin{tabular}{@{}c@{}}aTc\\~\end{tabular}}%
\psfrag{050}[tc][tc]{\matlabtextA }%
\psfrag{051}[bc][tc]{\matlabtextA \begin{tabular}{@{}c@{}c@{}}~\\LacI-TetR\\~\end{tabular}}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{7}{7}\selectfont\strut}%
\psfrag{000}[lt][rt]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $5$}%
\psfrag{002}[ct][ct]{\matlabtextB $10$}%
\psfrag{003}[ct][ct]{\matlabtextB $15$}%
\psfrag{004}[ct][ct]{\matlabtextB $20$}%
\psfrag{005}[ct][ct]{\matlabtextB $25$}%
\psfrag{006}[ct][ct]{\matlabtextB $30$}%
\psfrag{007}[ct][ct]{\matlabtextB $35$}%
\psfrag{008}[ct][ct]{\matlabtextB $40$}%
\psfrag{009}[ct][ct]{\matlabtextB $45$}%
\psfrag{014}[lt][rt]{\matlabtextB }%
\psfrag{015}[ct][ct]{\matlabtextB }%
\psfrag{016}[ct][ct]{\matlabtextB }%
\psfrag{017}[ct][ct]{\matlabtextB }%
\psfrag{018}[ct][ct]{\matlabtextB }%
\psfrag{019}[ct][ct]{\matlabtextB }%
\psfrag{020}[ct][ct]{\matlabtextB }%
\psfrag{021}[ct][ct]{\matlabtextB }%
\psfrag{022}[ct][ct]{\matlabtextB }%
\psfrag{023}[ct][ct]{\matlabtextB }%
\psfrag{028}[ct][ct]{\matlabtextB }%
\psfrag{029}[ct][ct]{\matlabtextB }%
\psfrag{030}[ct][ct]{\matlabtextB }%
\psfrag{031}[ct][ct]{\matlabtextB }%
\psfrag{032}[ct][ct]{\matlabtextB }%
\psfrag{033}[ct][ct]{\matlabtextB }%
\psfrag{034}[ct][ct]{\matlabtextB }%
\psfrag{035}[ct][ct]{\matlabtextB }%
\psfrag{036}[ct][ct]{\matlabtextB }%
\psfrag{037}[ct][ct]{\matlabtextB }%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rb]{\matlabtextB $0$}%
\psfrag{011}[rc][rc]{\matlabtextB }%
\psfrag{012}[rc][rc]{\matlabtextB }%
\psfrag{013}[rc][rb]{\matlabtextB $0.6$}%
\psfrag{024}[rc][rb]{\matlabtextB $0$}%
\psfrag{025}[rc][rc]{\matlabtextB }%
\psfrag{026}[rc][rc]{\matlabtextB }%
\psfrag{027}[rc][rb]{\matlabtextB $60$}%
\psfrag{038}[rc][lc]{\matlabtextB $0$}%
\psfrag{039}[rc][rc]{\matlabtextB $0.5$}%
\psfrag{040}[rc][lb]{\matlabtextB $1$}%
\psfrag{041}[rc][rb]{\matlabtextB $1.5$}%
\psfrag{042}[rc][lb]{\matlabtextB $2$}%
\psfrag{043}[rc][rb]{\matlabtextB $2.5$}%
\psfrag{044}[rc][lb]{\matlabtextB $3$}%
\psfrag{045}[rc][rb]{\matlabtextB $3.5$}%
%
%% </ytick>

==> PIPWModeCLres.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{048}[tc][bl]{\matlabtextA Time (h)}%
\psfrag{049}[bc][bc]{\matlabtextA 
\begin{tabular}{@{}c@{}c@{}} Duty\\Cycle\\~\end{tabular}}%
\psfrag{050}[tc][tc]{\matlabtextA }%
\psfrag{051}[bc][bc]{\matlabtextA \begin{tabular}{@{}c@{}}aTc\\~\end{tabular}}%
\psfrag{052}[tc][tc]{\matlabtextA }%
\psfrag{053}[bc][bc]{\matlabtextA \begin{tabular}{@{}c@{}}IPTG\\~\end{tabular}}%
\psfrag{054}[tc][tc]{\matlabtextA}%
\psfrag{055}[bc][bc]{\matlabtextA   \begin{tabular}{@{}c@{}}LacI-TetR\\~\end{tabular}}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{7}{7}\selectfont\strut}%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{6}{6}\selectfont\strut}%
\psfrag{000}[lt][rt]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $10$}%
\psfrag{002}[ct][ct]{\matlabtextC $20$}%
\psfrag{003}[ct][ct]{\matlabtextC $30$}%
\psfrag{004}[ct][ct]{\matlabtextC $40$}%
\psfrag{005}[ct][ct]{\matlabtextC $50$}%
\psfrag{006}[ct][ct]{\matlabtextC $60$}%
\psfrag{007}[ct][ct]{\matlabtextC $70$}%
\psfrag{011}[ct][rt]{\matlabtextC }%
\psfrag{012}[ct][ct]{\matlabtextC }%
\psfrag{013}[ct][ct]{\matlabtextC }%
\psfrag{014}[ct][ct]{\matlabtextC }%
\psfrag{015}[ct][ct]{\matlabtextC }%
\psfrag{016}[ct][ct]{\matlabtextC }%
\psfrag{017}[ct][ct]{\matlabtextC }%
\psfrag{018}[ct][ct]{\matlabtextC }%
\psfrag{022}[ct][rt]{\matlabtextC }%
\psfrag{023}[ct][ct]{\matlabtextC }%
\psfrag{024}[ct][ct]{\matlabtextC }%
\psfrag{025}[ct][ct]{\matlabtextC }%
\psfrag{026}[ct][ct]{\matlabtextC }%
\psfrag{027}[ct][ct]{\matlabtextC }%
\psfrag{028}[ct][ct]{\matlabtextC }%
\psfrag{029}[ct][ct]{\matlabtextC }%
\psfrag{033}[ct][rt]{\matlabtextC }%
\psfrag{034}[ct][ct]{\matlabtextC }%
\psfrag{035}[ct][ct]{\matlabtextC }%
\psfrag{036}[ct][ct]{\matlabtextC }%
\psfrag{037}[ct][ct]{\matlabtextC }%
\psfrag{038}[ct][ct]{\matlabtextC }%
\psfrag{039}[ct][ct]{\matlabtextC }%
\psfrag{040}[ct][ct]{\matlabtextC }%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{008}[rc][rb]{\matlabtextB $0$}%
\psfrag{009}[rc][rb]{\matlabtextB }%$0.5$}%
\psfrag{010}[rc][rb]{\matlabtextB $1$}%
\psfrag{019}[rc][rb]{\matlabtextB $0$}%
\psfrag{020}[rc][rb]{\matlabtextB }%$20$}%
\psfrag{021}[rc][rb]{\matlabtextB $40$}%
\psfrag{030}[rc][rb]{\matlabtextB $0$}%
\psfrag{031}[rc][rb]{\matlabtextB }%$0.2$}%
\psfrag{032}[rc][rb]{\matlabtextB $0.4$}%
\psfrag{041}[rc][cc]{\matlabtextB $0$}%
\psfrag{042}[rc][rc]{\matlabtextB $0.5$}%
\psfrag{043}[rc][cb]{\matlabtextB $1$}%
\psfrag{044}[rc][rb]{\matlabtextB $1.5$}%
\psfrag{045}[rc][cb]{\matlabtextB $2$}%
\psfrag{046}[rc][rb]{\matlabtextB $2.5$}%
\psfrag{047}[rc][cb]{\matlabtextB $3$}%
%
%% </ytick>

==> PIPWModeOLres.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{048}[tc][bc]{\matlabtextA Time (h)}%
\psfrag{049}[bc][bc]{\matlabtextA 
\begin{tabular}{@{}c@{}c@{}} Duty\\Cycle\\~\end{tabular}}%
\psfrag{050}[tc][tc]{\matlabtextA }%
\psfrag{051}[bc][bc]{\matlabtextA \begin{tabular}{@{}c@{}}aTc\\~\end{tabular}}%
\psfrag{052}[tc][tc]{\matlabtextA }%
\psfrag{053}[bc][bc]{\matlabtextA \begin{tabular}{@{}c@{}}IPTG\\~\end{tabular}}%
\psfrag{054}[tc][tc]{\matlabtextA}%
\psfrag{055}[bc][bc]{\matlabtextA   \begin{tabular}{@{}c@{}}LacI-TetR\\~\end{tabular}}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{7}{7}\selectfont\strut}%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{6}{6}\selectfont\strut}%
\psfrag{000}[lt][rt]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $10$}%
\psfrag{002}[ct][ct]{\matlabtextC $20$}%
\psfrag{003}[ct][ct]{\matlabtextC $30$}%
\psfrag{004}[ct][ct]{\matlabtextC $40$}%
\psfrag{005}[ct][ct]{\matlabtextC $50$}%
\psfrag{006}[ct][ct]{\matlabtextC $60$}%
\psfrag{007}[ct][ct]{\matlabtextC $70$}%
\psfrag{011}[ct][rt]{\matlabtextC }%
\psfrag{012}[ct][ct]{\matlabtextC }%
\psfrag{013}[ct][ct]{\matlabtextC }%
\psfrag{014}[ct][ct]{\matlabtextC }%
\psfrag{015}[ct][ct]{\matlabtextC }%
\psfrag{016}[ct][ct]{\matlabtextC }%
\psfrag{017}[ct][ct]{\matlabtextC }%
\psfrag{018}[ct][ct]{\matlabtextC }%
\psfrag{022}[ct][rt]{\matlabtextC }%
\psfrag{023}[ct][ct]{\matlabtextC }%
\psfrag{024}[ct][ct]{\matlabtextC }%
\psfrag{025}[ct][ct]{\matlabtextC }%
\psfrag{026}[ct][ct]{\matlabtextC }%
\psfrag{027}[ct][ct]{\matlabtextC }%
\psfrag{028}[ct][ct]{\matlabtextC }%
\psfrag{029}[ct][ct]{\matlabtextC }%
\psfrag{033}[ct][rt]{\matlabtextC }%
\psfrag{034}[ct][ct]{\matlabtextC }%
\psfrag{035}[ct][ct]{\matlabtextC }%
\psfrag{036}[ct][ct]{\matlabtextC }%
\psfrag{037}[ct][ct]{\matlabtextC }%
\psfrag{038}[ct][ct]{\matlabtextC }%
\psfrag{039}[ct][ct]{\matlabtextC }%
\psfrag{040}[ct][ct]{\matlabtextC }%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{008}[rc][rb]{\matlabtextB $0$}%
\psfrag{009}[rc][rb]{\matlabtextB }%$0.5$}%
\psfrag{010}[rc][rb]{\matlabtextB $1$}%
\psfrag{019}[rc][rb]{\matlabtextB $0$}%
\psfrag{020}[rc][rb]{\matlabtextB }%$20$}%
\psfrag{021}[rc][rb]{\matlabtextB $40$}%
\psfrag{030}[rc][rb]{\matlabtextB $0$}%
\psfrag{031}[rc][rb]{\matlabtextB }%$0.2$}%
\psfrag{032}[rc][rb]{\matlabtextB $0.4$}%
\psfrag{041}[rc][cc]{\matlabtextB $0$}%
\psfrag{042}[rc][rb]{\matlabtextB $0.5$}%
\psfrag{043}[rc][cb]{\matlabtextB $1$}%
\psfrag{044}[rc][rb]{\matlabtextB $1.5$}%
\psfrag{045}[rc][cb]{\matlabtextB $2$}%
\psfrag{046}[rc][rb]{\matlabtextB $2.5$}%
\psfrag{047}[rc][cb]{\matlabtextB $3$}%
%
%% </ytick>

==> PIPWMssaCLres.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{049}[tc][tc]{\matlabtextA Time (h)}%
\psfrag{050}[bc][bc]{\matlabtextA 
\begin{tabular}{@{}c@{}c@{}} ~\\Duty\\Cycle\end{tabular}}%
\psfrag{051}[tc][tc]{\matlabtextA }%
\psfrag{052}[bc][bc]{\matlabtextA aTc}%
\psfrag{053}[tc][tc]{\matlabtextA }%
\psfrag{054}[bc][bc]{\matlabtextA IPTG}%
\psfrag{055}[tc][tc]{\matlabtextA}%
\psfrag{056}[ct][cb]{\matlabtextA LacI-TetR}
%\psfrag{056}[bl][bc]{\matlabtextA \begin{tabular}{@{}c@{}} ~\\LacI-TetR\end{tabular}}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{7}{7}\selectfont\strut}%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{6}{6}\selectfont\strut}%
\providecommand\matlabtextD{\color[rgb]{0.150,0.150,0.150}\fontsize{5}{5}\selectfont\strut}%
\psfrag{000}[lt][rt]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $10$}%
\psfrag{002}[ct][ct]{\matlabtextC $20$}%
\psfrag{003}[ct][ct]{\matlabtextC $30$}%
\psfrag{004}[ct][ct]{\matlabtextC $40$}%
\psfrag{005}[ct][ct]{\matlabtextC $50$}%
\psfrag{006}[ct][ct]{\matlabtextC $60$}%
\psfrag{007}[ct][ct]{\matlabtextC $70$}%
\psfrag{011}[ct][rt]{\matlabtextC }%
\psfrag{012}[ct][ct]{\matlabtextD }%
\psfrag{013}[ct][ct]{\matlabtextD }%
\psfrag{014}[ct][ct]{\matlabtextD }%
\psfrag{015}[ct][ct]{\matlabtextD }%
\psfrag{016}[ct][ct]{\matlabtextD }%
\psfrag{017}[ct][ct]{\matlabtextD }%
\psfrag{018}[ct][ct]{\matlabtextD }%
\psfrag{022}[ct][rt]{\matlabtextC }%
\psfrag{023}[ct][ct]{\matlabtextC }%
\psfrag{024}[ct][ct]{\matlabtextC }%
\psfrag{025}[ct][ct]{\matlabtextC }%
\psfrag{026}[ct][ct]{\matlabtextC }%
\psfrag{027}[ct][ct]{\matlabtextC }%
\psfrag{028}[ct][ct]{\matlabtextC }%
\psfrag{029}[ct][ct]{\matlabtextC }%
\psfrag{033}[ct][rt]{\matlabtextC }%
\psfrag{034}[ct][ct]{\matlabtextC }%
\psfrag{035}[ct][ct]{\matlabtextC }%
\psfrag{036}[ct][ct]{\matlabtextC }%
\psfrag{037}[ct][ct]{\matlabtextC }%
\psfrag{038}[ct][ct]{\matlabtextC }%
\psfrag{039}[ct][ct]{\matlabtextC }%
\psfrag{040}[ct][ct]{\matlabtextC }%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{008}[rc][rb]{\matlabtextB $0$}%
\psfrag{009}[rc][rb]{\matlabtextB }%$0.5$}%
\psfrag{010}[rc][rb]{\matlabtextB $1$}%
\psfrag{019}[rc][rb]{\matlabtextB $0$}%
\psfrag{020}[rc][rb]{\matlabtextB }%$20$}%
\psfrag{021}[rc][rb]{\matlabtextB $40$}%
\psfrag{030}[rc][rb]{\matlabtextB $0$}%
\psfrag{031}[rc][rb]{\matlabtextB }%$0.2$}%
\psfrag{032}[rc][rb]{\matlabtextB $0.4$}%
\psfrag{041}[rc][cc]{\matlabtextB $0$}%
\psfrag{042}[rc][rb]{\matlabtextB $0.5$}%
\psfrag{043}[rc][cb]{\matlabtextB $1$}%
\psfrag{044}[rc][rb]{\matlabtextB $1.5$}%
\psfrag{045}[rc][cb]{\matlabtextB $2$}%
\psfrag{046}[rc][rb]{\matlabtextB $2.5$}%
\psfrag{047}[rc][cb]{\matlabtextB $3$}%
\psfrag{048}[rc][rb]{\matlabtextB $3.5$}%
%
%% </ytick>

==> PIPWMssaMean.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{016}[tc][tc]{\matlabtextA \begin{tabular}{@{}c@{}c@{}}~\\Time (h)\\~\end{tabular}}%
\psfrag{017}[bc][tc]{\matlabtextA \begin{tabular}{@{}c@{}}~\\LacI-TetR\\~\end{tabular}}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{7}{7}\selectfont\strut}%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{6}{6}\selectfont\strut}%
\psfrag{000}[ct][rt]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $10$}%
\psfrag{002}[ct][ct]{\matlabtextC $20$}%
\psfrag{003}[ct][ct]{\matlabtextC $30$}%
\psfrag{004}[ct][ct]{\matlabtextC $40$}%
\psfrag{005}[ct][ct]{\matlabtextC $50$}%
\psfrag{006}[ct][ct]{\matlabtextC $60$}%
\psfrag{007}[ct][ct]{\matlabtextC $70$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{008}[rc][cc]{\matlabtextB $0$}%
\psfrag{009}[rc][rb]{\matlabtextB $0.5$}%
\psfrag{010}[rc][cb]{\matlabtextB $1$}%
\psfrag{011}[rc][rb]{\matlabtextB $1.5$}%
\psfrag{012}[rc][cb]{\matlabtextB $2$}%
\psfrag{013}[rc][rb]{\matlabtextB $2.5$}%
\psfrag{014}[rc][cb]{\matlabtextB $3$}%
\psfrag{015}[rc][rb]{\matlabtextB $3.5$}%
%
%% </ytick>

==> PIPopAvgNoSW2.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{8}\selectfont\strut}%
\psfrag{043}[tc][tc]{\matlabtextA \begin{tabular}{@{}c@{}}~\\Time (h)\end{tabular}}%
\psfrag{044}[bc][bc]{\matlabtextA \begin{tabular}{@{}c@{}}aTc\\~\end{tabular}}%
\psfrag{045}[tc][tc]{\matlabtextA }%
\psfrag{046}[bc][bc]{\matlabtextA \begin{tabular}{@{}c@{}}IPTG\\~\end{tabular}}%
\psfrag{047}[tc][tc]{\matlabtextA }%
\psfrag{048}[bc][bc]{\matlabtextA \begin{tabular}{@{}c@{}c@{}}~\\LacI-TetR\\~\end{tabular}}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{7}{7}\selectfont\strut}%
\psfrag{000}[lt][rt]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $5$}%
\psfrag{002}[ct][ct]{\matlabtextB $10$}%
\psfrag{003}[ct][ct]{\matlabtextB $15$}%
\psfrag{004}[ct][ct]{\matlabtextB $20$}%
\psfrag{005}[ct][ct]{\matlabtextB $25$}%
\psfrag{006}[ct][ct]{\matlabtextB $30$}%
\psfrag{007}[ct][ct]{\matlabtextB $35$}%
\psfrag{008}[ct][ct]{\matlabtextB $40$}%
\psfrag{009}[ct][ct]{\matlabtextB $45$}%
\psfrag{012}[ct][rt]{\matlabtextB }%
\psfrag{013}[ct][ct]{\matlabtextB }%
\psfrag{014}[ct][ct]{\matlabtextB }%
\psfrag{015}[ct][ct]{\matlabtextB }%
\psfrag{016}[ct][ct]{\matlabtextB }%
\psfrag{017}[ct][ct]{\matlabtextB }%
\psfrag{018}[ct][ct]{\matlabtextB }%
\psfrag{019}[ct][ct]{\matlabtextB }%
\psfrag{020}[ct][ct]{\matlabtextB }%
\psfrag{021}[ct][ct]{\matlabtextB }%
\psfrag{025}[ct][rt]{\matlabtextB }%
\psfrag{026}[ct][ct]{\matlabtextB }%
\psfrag{027}[ct][ct]{\matlabtextB }%
\psfrag{028}[ct][ct]{\matlabtextB }%
\psfrag{029}[ct][ct]{\matlabtextB }%
\psfrag{030}[ct][ct]{\matlabtextB }%
\psfrag{031}[ct][ct]{\matlabtextB }%
\psfrag{032}[ct][ct]{\matlabtextB }%
\psfrag{033}[ct][ct]{\matlabtextB }%
\psfrag{034}[ct][ct]{\matlabtextB }%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rb]{\matlabtextB $0$}%
\psfrag{011}[rc][rb]{\matlabtextB $50$}%
\psfrag{022}[rc][rb]{\matlabtextB $0$}%
\psfrag{023}[rc][rb]{\matlabtextB $0.2$}%
\psfrag{024}[rc][rb]{\matlabtextB $0.4$}%
\psfrag{035}[rc][cc]{\matlabtextB $0$}%
\psfrag{036}[rc][rc]{\matlabtextB $0.5$}%
\psfrag{037}[rc][cb]{\matlabtextB $1$}%
\psfrag{038}[rc][rb]{\matlabtextB $1.5$}%
\psfrag{039}[rc][cb]{\matlabtextB $2$}%
\psfrag{040}[rc][rb]{\matlabtextB $2.5$}%
\psfrag{041}[rc][cb]{\matlabtextB $3$}%
\psfrag{042}[rc][rb]{\matlabtextB $3.5$}%
%
%% </ytick>

==> ZADodeDIFF.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{047}[tc][tc]{\matlabtextA \begin{tabular}{@{}c@{}}~\\Time (h)\end{tabular}}%
\psfrag{048}[bc][bc]{\matlabtextA \begin{tabular}{@{}c@{}c@{}}Duty\\Cycle\\~\end{tabular}}%
\psfrag{049}[tc][tc]{\matlabtextA }%
\psfrag{050}[bc][bc]{\matlabtextA \begin{tabular}{@{}c@{}}aTc\\~\end{tabular}}%
\psfrag{051}[tc][tc]{\matlabtextA }%
\psfrag{052}[bc][bc]{\matlabtextA \begin{tabular}{@{}c@{}}IPTG\\~\end{tabular}}%
\psfrag{053}[tc][tc]{\matlabtextA }%
\psfrag{054}[bc][bc]{\matlabtextA  \begin{tabular}{@{}c@{}}LacI-TetR\\~\end{tabular}}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{6}{6}\selectfont\strut}%
\psfrag{000}[lt][rt]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $10$}%
\psfrag{002}[ct][ct]{\matlabtextB $20$}%
\psfrag{003}[ct][ct]{\matlabtextB $30$}%
\psfrag{004}[ct][ct]{\matlabtextB $40$}%
\psfrag{005}[ct][ct]{\matlabtextB $50$}%
\psfrag{006}[ct][ct]{\matlabtextB $60$}%
\psfrag{007}[ct][ct]{\matlabtextB $70$}%
\psfrag{011}[ct][ct]{\matlabtextB }%
\psfrag{012}[ct][ct]{\matlabtextB }%
\psfrag{013}[ct][ct]{\matlabtextB }%
\psfrag{014}[ct][ct]{\matlabtextB }%
\psfrag{015}[ct][ct]{\matlabtextB }%
\psfrag{016}[ct][ct]{\matlabtextB }%
\psfrag{017}[ct][ct]{\matlabtextB }%
\psfrag{018}[ct][ct]{\matlabtextB }%
\psfrag{021}[ct][ct]{\matlabtextB }%
\psfrag{022}[ct][ct]{\matlabtextB }%
\psfrag{023}[ct][ct]{\matlabtextB }%
\psfrag{024}[ct][ct]{\matlabtextB }%
\psfrag{025}[ct][ct]{\matlabtextB }%
\psfrag{026}[ct][ct]{\matlabtextB }%
\psfrag{027}[ct][ct]{\matlabtextB }%
\psfrag{028}[ct][ct]{\matlabtextB }%
\psfrag{031}[ct][ct]{\matlabtextB }%
\psfrag{032}[ct][ct]{\matlabtextB }%
\psfrag{033}[ct][ct]{\matlabtextB }%
\psfrag{034}[ct][ct]{\matlabtextB }%
\psfrag{035}[ct][ct]{\matlabtextB }%
\psfrag{036}[ct][ct]{\matlabtextB }%
\psfrag{037}[ct][ct]{\matlabtextB }%
\psfrag{038}[ct][ct]{\matlabtextB }%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{008}[rc][rc]{\matlabtextB $0$}%
\psfrag{009}[rc][rc]{\matlabtextB $0.5$}%
\psfrag{010}[rc][rc]{\matlabtextB $1$}%
\psfrag{019}[rc][rc]{\matlabtextB $0$}%
\psfrag{020}[rt][rb]{\matlabtextB $60$}%
\psfrag{029}[rc][rc]{\matlabtextB $0$}%
\psfrag{030}[rt][rb]{\matlabtextB $0.6$}%
\psfrag{039}[rc][lc]{\matlabtextB $0$}%
\psfrag{040}[rc][rc]{\matlabtextB $0.5$}%
\psfrag{041}[rc][lc]{\matlabtextB $1$}%
\psfrag{042}[rc][rc]{\matlabtextB $1.5$}%
\psfrag{043}[rc][lc]{\matlabtextB $2$}%
\psfrag{044}[rc][rc]{\matlabtextB $2.5$}%
\psfrag{045}[rc][lc]{\matlabtextB $3$}%
\psfrag{046}[rc][rc]{\matlabtextB $3.5$}%
%
%% </ytick>

==> ZADodeNODIFF.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{047}[tc][tc]{\matlabtextA \begin{tabular}{@{}c@{}}~\\Time (h)\end{tabular}}%
\psfrag{048}[bc][bc]{\matlabtextA \begin{tabular}{@{}c@{}c@{}}Duty\\Cycle\\~\end{tabular}}%
\psfrag{049}[tc][tc]{\matlabtextA }%
\psfrag{050}[bc][bc]{\matlabtextA \begin{tabular}{@{}c@{}}aTc\\~\end{tabular}}%
\psfrag{051}[tc][tc]{\matlabtextA }%
\psfrag{052}[bc][bc]{\matlabtextA \begin{tabular}{@{}c@{}}IPTG\\~\end{tabular}}%
\psfrag{053}[tc][tc]{\matlabtextA }%
\psfrag{054}[bc][bc]{\matlabtextA  \begin{tabular}{@{}c@{}}LacI-TetR\\~\end{tabular}}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{6}{6}\selectfont\strut}%
\psfrag{000}[lt][rt]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $10$}%
\psfrag{002}[ct][ct]{\matlabtextB $20$}%
\psfrag{003}[ct][ct]{\matlabtextB $30$}%
\psfrag{004}[ct][ct]{\matlabtextB $40$}%
\psfrag{005}[ct][ct]{\matlabtextB $50$}%
\psfrag{006}[ct][ct]{\matlabtextB $60$}%
\psfrag{007}[ct][ct]{\matlabtextB $70$}%
\psfrag{011}[ct][ct]{\matlabtextB }%
\psfrag{012}[ct][ct]{\matlabtextB }%
\psfrag{013}[ct][ct]{\matlabtextB }%
\psfrag{014}[ct][ct]{\matlabtextB }%
\psfrag{015}[ct][ct]{\matlabtextB }%
\psfrag{016}[ct][ct]{\matlabtextB }%
\psfrag{017}[ct][ct]{\matlabtextB }%
\psfrag{018}[ct][ct]{\matlabtextB }%
\psfrag{021}[ct][ct]{\matlabtextB }%
\psfrag{022}[ct][ct]{\matlabtextB }%
\psfrag{023}[ct][ct]{\matlabtextB }%
\psfrag{024}[ct][ct]{\matlabtextB }%
\psfrag{025}[ct][ct]{\matlabtextB }%
\psfrag{026}[ct][ct]{\matlabtextB }%
\psfrag{027}[ct][ct]{\matlabtextB }%
\psfrag{028}[ct][ct]{\matlabtextB }%
\psfrag{031}[ct][ct]{\matlabtextB }%
\psfrag{032}[ct][ct]{\matlabtextB }%
\psfrag{033}[ct][ct]{\matlabtextB }%
\psfrag{034}[ct][ct]{\matlabtextB }%
\psfrag{035}[ct][ct]{\matlabtextB }%
\psfrag{036}[ct][ct]{\matlabtextB }%
\psfrag{037}[ct][ct]{\matlabtextB }%
\psfrag{038}[ct][ct]{\matlabtextB }%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{008}[rc][rb]{\matlabtextB $0$}%
\psfrag{009}[rc][rb]{\matlabtextB $0.5$}%
\psfrag{010}[rc][rb]{\matlabtextB $1$}%
\psfrag{019}[rc][rb]{\matlabtextB $0$}%
\psfrag{020}[rt][rb]{\matlabtextB $60$}%
\psfrag{029}[rc][rb]{\matlabtextB $0$}%
\psfrag{030}[rt][rb]{\matlabtextB $0.6$}%
\psfrag{039}[rc][cc]{\matlabtextB $0$}%
\psfrag{040}[rc][rb]{\matlabtextB $0.5$}%
\psfrag{041}[rc][lb]{\matlabtextB $1$}%
\psfrag{042}[rc][rb]{\matlabtextB $1.5$}%
\psfrag{043}[rc][lb]{\matlabtextB $2$}%
\psfrag{044}[rc][rb]{\matlabtextB $2.5$}%
\psfrag{045}[rc][lb]{\matlabtextB $3$}%
\psfrag{046}[rc][rb]{\matlabtextB $3.5$}%

%
%% </ytick>

==> ZADssaNODIFF.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{048}[tc][tc]{\matlabtextA \begin{tabular}{@{}c@{}}~\\Time (h)\end{tabular}}%
\psfrag{049}[bc][bc]{\matlabtextA \begin{tabular}{@{}c@{}c@{}}Duty\\Cycle\\~\end{tabular}}%
\psfrag{050}[tc][tc]{\matlabtextA }%
\psfrag{051}[bc][bc]{\matlabtextA \begin{tabular}{@{}c@{}}aTc\\~\end{tabular}}%
\psfrag{052}[tc][tc]{\matlabtextA }%
\psfrag{053}[bc][bc]{\matlabtextA \begin{tabular}{@{}c@{}}IPTG\\~\end{tabular}}%
\psfrag{054}[tc][tc]{\matlabtextA }%
\psfrag{055}[bc][bc]{\matlabtextA  \begin{tabular}{@{}c@{}}LacI-TetR\\~\end{tabular}}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{6}{6}\selectfont\strut}%
\psfrag{000}[lt][rt]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $10$}%
\psfrag{002}[ct][ct]{\matlabtextB $20$}%
\psfrag{003}[ct][ct]{\matlabtextB $30$}%
\psfrag{004}[ct][ct]{\matlabtextB $40$}%
\psfrag{005}[ct][ct]{\matlabtextB $50$}%
\psfrag{006}[ct][ct]{\matlabtextB $60$}%
\psfrag{007}[ct][ct]{\matlabtextB $70$}%
\psfrag{011}[ct][rt]{\matlabtextB }%
\psfrag{012}[ct][ct]{\matlabtextB }%
\psfrag{013}[ct][ct]{\matlabtextB }%
\psfrag{014}[ct][ct]{\matlabtextB }%
\psfrag{015}[ct][ct]{\matlabtextB }%
\psfrag{016}[ct][ct]{\matlabtextB }%
\psfrag{017}[ct][ct]{\matlabtextB }%
\psfrag{018}[ct][ct]{\matlabtextB }%
\psfrag{021}[ct][rt]{\matlabtextB }%
\psfrag{022}[ct][ct]{\matlabtextB }%
\psfrag{023}[ct][ct]{\matlabtextB }%
\psfrag{024}[ct][ct]{\matlabtextB }%
\psfrag{025}[ct][ct]{\matlabtextB }%
\psfrag{026}[ct][ct]{\matlabtextB }%
\psfrag{027}[ct][ct]{\matlabtextB }%
\psfrag{028}[ct][ct]{\matlabtextB }%
\psfrag{031}[ct][rt]{\matlabtextB }%
\psfrag{032}[ct][ct]{\matlabtextB }%
\psfrag{033}[ct][ct]{\matlabtextB }%
\psfrag{034}[ct][ct]{\matlabtextB }%
\psfrag{035}[ct][ct]{\matlabtextB }%
\psfrag{036}[ct][ct]{\matlabtextB }%
\psfrag{037}[ct][ct]{\matlabtextB }%
\psfrag{038}[ct][ct]{\matlabtextB }%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{008}[rc][rb]{\matlabtextB $0$}%
\psfrag{009}[rc][rb]{\matlabtextB $0.5$}%
\psfrag{010}[rc][rb]{\matlabtextB $1$}%
\psfrag{019}[rc][rb]{\matlabtextB $0$}%
\psfrag{020}[rt][rb]{\matlabtextB $60$}%
\psfrag{029}[rc][rb]{\matlabtextB $0$}%
\psfrag{030}[rt][rb]{\matlabtextB $0.6$}%
\psfrag{039}[rc][lc]{\matlabtextB $0$}%
\psfrag{040}[rc][rb]{\matlabtextB $0.5$}%
\psfrag{041}[rc][lb]{\matlabtextB $1$}%
\psfrag{042}[rc][rb]{\matlabtextB $1.5$}%
\psfrag{043}[rc][lb]{\matlabtextB $2$}%
\psfrag{044}[rc][rb]{\matlabtextB $2.5$}%
\psfrag{045}[rc][lb]{\matlabtextB $3$}%
\psfrag{046}[rc][rb]{\matlabtextB $3.5$}%
\psfrag{047}[rc][lb]{\matlabtextB $4$}%
%
%% </ytick>
